Anomaly Detection and Failure Root Cause Analysis in (Micro)Service-Based Cloud Applications: A Survey

The momentum gained by microservices and cloud-native software architecture pushed nowadays enterprise IT towards multi-service applications. The proliferation of services and service interactions within applications, often consisting of hundreds of interacting services, makes it harder to detect failures and to identify their possible root causes, which is on the other hand crucial to promptly recover and fix applications. Various techniques have been proposed to promptly detect failures based on their symptoms, viz., observing anomalous behaviour in one or more application services, as well as to analyse logs or monitored performance of such services to determine the possible root causes for observed anomalies. The objective of this survey is to provide a structured overview and a qualitative analysis of currently available techniques for anomaly detection and root cause analysis in modern multi-service applications. Some open challenges and research directions stemming out from the analysis are also discussed.

==> tab/detection.tex <==
\begin{table}[tp]
\caption{Classification of anomaly detection techniques, based on their \textit{class} (\viz \textsf{L}, \textsf{DT}, and \textsf{M} for log-based, distributed tracing-based, and monitoring-based techniques, respectively), the applied \textit{method}, the \textit{type} (\viz \textsf{F} and \textsf{P} for functional and performance anomalies, respectively) and \textit{granularity} of detected anomalies (\viz \textsf{A} and \textsf{S} for application-level and service-level anomalies, respectively), and the \textit{artifacts} they need to run.}
\label{tab:detection}
\begin{footnotesize}
\begin{tabular}{%
    >{\centering\arraybackslash}m{.2\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.06\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.21\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.05\textwidth}%
    @{\,}
    >{\centering\arraybackslash}m{.11\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.32\textwidth}%
}
    \thickline
    %study
        & 
        &
        & \multicolumn{2}{c}{\textbf{Anomaly}}
        & 
        \\ 
    %study
        & \textbf{Class} 
        & \textbf{Detection Method}
        & \textbf{Type}
        & \textbf{Granularity} 
        & \textbf{Needed Artifacts}
        \\ 
    \thickline
    OASIS \cite{38_Nandi2016_AnomalyDetectionControlFlowGraphMining}
        & \textsf{L} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{F}
        & \textsf{A}
        & training logs, runtime logs
        \\
    Jia \etal \cite{31_Jia2017_AnomalyDiagnosisHybridGraphModel}
        & \textsf{L} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & training logs, runtime logs
        \\
    LogSed \cite{32_Jia2017_LogSed}
        & \textsf{L} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & training logs, runtime logs
        \\
        \thinline
    TraceAnomaly \cite{16_Liu2020_TraceAnomaly}
        & \textsf{DT} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & training traces, runtime traces
        \\
    Nedelkoski \etal \cite{35_Nedelkoski2019_AnomalyDetectionTracingData}
        & \textsf{DT}  %(with Zipkin
        & \cellcolor[HTML]{FDF3ED} unsupervised learning 
        %& online
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & training traces, runtime traces
        \\
    Jin \etal \cite{22_Jin2020_AnomalyDetectionMicroservicesRPCA}
        & \textsf{DT} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning 
        %& offline % the authors explicitly state that their approach works well only offline
        & \textsf{P}
        & \textsf{S}
        & reference traces, runtime traces
        \\
    
    Seer \cite{17_Gan2019_Seer}
        & \textsf{DT} 
        & \cellcolor[HTML]{D9FDE5} supervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & training traces, runtime traces
        \\
    
    Nedelkoski \etal \cite{34_Nedelkoski2019_AnomalyDetectionDistributedTracing}
        & \textsf{DT}  %(with Zipkin
        & \cellcolor[HTML]{D9FDE5} supervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & training traces, runtime traces
        \\
    
    Bogatinovski \etal \cite{36_Bogatinovski2020_SelfSupervisedAnomalyDetection}
        & \textsf{DT} 
        & \cellcolor[HTML]{D9FDE5} supervised learning
        & \textsf{P}
        & \textsf{A}
        & training traces, runtime traces
        \\
    
    MEPFL \cite{02_Zhou2019_LatentErrorPrediction}
        & \textsf{DT} 
        & \cellcolor[HTML]{D9FDE5} supervised learning 
        %& online               
        & \textsf{F}
        & \textsf{S}
        & target application deployment, automated test cases
        \\
    Meng \etal \cite{23_Meng2021_DetectingAnomaliesMicroservices}
        & \textsf{DT}  %(with Jaeger, Zipkin
        & \cellcolor[HTML]{dce3ac} trace comparison
        %& offline % in TTV, authors state that the proposed approach is too costly to enact online detection on medium/large-scale multi-service apps
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & reference traces, runtime traces
        \\
    Wang \etal \cite{26_Wang2020_WorkflowAwareFaultDiagnosis}
        & \textsf{DT}  %(with OpenTracing
        & \cellcolor[HTML]{dce3ac} trace comparison
        %& offline % in TTV, authors state that the proposed approach is too costly to enact online detection on medium/large-scale multi-service apps
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & reference traces, runtime traces
        \\
    Chen \etal \cite{39_Chen2020_MatrixSketchBasedAnomalyDetection}
        & \textsf{DT} 
        & \cellcolor[HTML]{dce3ac} trace comparison
        %& online
        & \textsf{P}
        & \textsf{S}
        & reference traces, runtime traces
        \\
        \thinline
    Gulenko \etal \cite{37_Gulenko2018_DetectingAnomalousBehaviourBlackBoxServices}
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & target application deployment, workload generator
        \\
    LOUD \cite{13_Mariani2018_LocalizingFaultsCloudSystems}
        & \textsf{M}  
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & target application deployment, workload generator
        \\
    MicroRCA \cite{04_Wu2020_MicroRCA} 
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & k8s deployment, workload generator
        \\ 
    
    Wu \etal \cite{09_Wu2020_MicroserviceDiagnosisDeepLearning}
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & k8s deployment, workload generator
        \\
    
    DLA \cite{14_Samir2019_DLA}
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & k8s deployment % HHMM model - not for anomaly detection!
        \\
    
    CloudRanger \cite{29_Wang2018_CloudRanger}
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{A}
        & target application deployment, historically monitored KPIs
        \\
    
    Hora \cite{27_Pitakrat2018_HoraExtended,28_Pitakrat2016_Hora}
        & \textsf{M} 
        & \cellcolor[HTML]{FDF3ED} unsupervised learning
        %& online
        & \textsf{P}
        & \textsf{S}
        & target application deployment
        \\
    ADS \cite{15_Du2018_AnomalyDetectionContainerMicroservices}
        & \textsf{M} 
        & \cellcolor[HTML]{D9FDE5} supervised learning
        & \textsf{P}
        & \textsf{S}
        & k8s deployment, failure injectors, workload generator
        \\
    PreMiSE \cite{33_Mariani2020_PredictingFailures}
        & \textsf{M} 
        & \cellcolor[HTML]{D9FDE5} supervised learning
        %& online
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & target application deployment, workload generator % with one service per VM
        \\
    
    CauseInfer \cite{40_Chen2020_CauseInfer,48_Chen2014_CauseInfer}
        & \textsf{M} 
        & \cellcolor[HTML]{d1bfb3} SLO check
        %& online
        & \textsf{P}
        & \textsf{A}
        & target application deployment, SLOs
        \\
    
    MicroScope \cite{06_Lin2018_Microscope,19_Guan2019_MicroscopeDemo}
        & \textsf{M} %\textsf{M} 
        & \cellcolor[HTML]{d1bfb3} SLO check
        %& online
        & \textsf{P}
        & \textsf{A}
        & k8s deployment, SLOs
        \\
    
    $\epsilon$-diagnosis \cite{49_Shan2019_epsilonDiagnosis}
        & \textsf{M} 
        & \cellcolor[HTML]{d1bfb3} SLO check
        %& online
        & \textsf{P}
        & \textsf{A}
        & k8s deployment, SLOs
        \\
    M-MFSA- HDA \cite{24_Zang2018_FaultDiagnosisMicroservices}
        & \textsf{M} 
        & \cellcolor[HTML]{7BE0C5} heartbeating
        %& online
        & \textsf{F}
        & \textsf{S}
        & target application deployment
        \\
    \thickline
\end{tabular}
\end{footnotesize}
\end{table}

==> tab/old/rca-old.tex <==
\begin{table}[tp]
\caption{Classification of root cause analysis techniques, based on their \textit{class} (\viz \textsf{L}, \textsf{DT}, and \textsf{M} for log-based, distributed tracing-based, and monitoring-based techniques, respectively), the enacted \textit{search}, the \textit{type} (\viz \textsf{F} and \textsf{P} for functional and performance anomalies, respectively) and \textit{grain} of explained anomalies (\viz \textsf{A} and \textsf{S} for application-level and service-level anomalies, respectively), the identified \textit{root causes}, and the \textit{artifacts} they need to run. The techniques marked with \enquote{${}^\star$} automatically enact root cause analysis for anomalies they automatically detect on running applications (as described in \Cref{sec:detection}). }
\label{tab:rca}
\begin{footnotesize}
\begin{tabular}{%
    >{\centering\arraybackslash}m{.18\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.05\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.16\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.05\textwidth}%
    @{\,}
    >{\centering\arraybackslash}m{.06\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.18\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.25\textwidth}%
}
    \thickline
    % study
        &
        &
        & \multicolumn{2}{c}{\textbf{Anomaly}}
        &
        &
        \\
    %study
        & \textbf{Class} 
        & \textbf{Analysis Method}
        & \textbf{Type}
        & \textbf{Gran.}
        & \textbf{Root Causes}
        & \textbf{Needed Artifacts}
        \\ 
    \thickline
    Aggarwal \etal \cite{10_Aggarwal2020_FaultsGoldenSignals}
        & \textsf{L}
        & \cellcolor[HTML]{eeeeee} \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{F}
        & \textsf{A}
        & service
        & online produced logs, application specification
        \\
    \thinline
    Zhou \etal \cite{01_Zhou2021_FaultAnalysisDebuggingMicroservices}
        & \textsf{DT}
        & \cellcolor[HTML]{dddddd} trace comparison
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & set of trace events 
        & reference traces, online produced traces
        \\
    GMTA \cite{45_Guo2020_GMTA}
        & \textsf{DT}
        & \cellcolor[HTML]{dddddd} trace comparison
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & set of services
        & reference traces, online produced traces
        \\
    
    CloudDiag \cite{41_Mi2013_PerformanceDiagnosisCloud}
        & \textsf{DT}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment
        \\
    
    ${}^\star$TraceAnomaly \cite{16_Liu2020_TraceAnomaly}
        & \textsf{DT}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & set of services
        & training traces, online produced traces
        \\
    MonitorRank \cite{21_Kim2013_RootCauseDetectionSOA}
        & \textsf{DT}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment
        \\
    MicroHECL \cite{47_Liu2021_MicroHECL}
        & \textsf{DT}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{S}
        & ranked list of services
        & training traces, online produced traces
        \\
    \thinline
    ${}^\star \epsilon$-diagnosis \cite{49_Shan2019_epsilonDiagnosis}
        & \textsf{M}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{P}
        & \textsf{A}
        & set of KPIs
        & k8s deployment
        \\
    
    ${}^\star$Wang \etal \cite{20_Wang2020_RootCauseMetricLocation}
        & \textsf{M}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & set of KPIs
        & online produced logs, monitored KPIs
        \\
    
    PAL \cite{42_Nguyen2011_PAL}
        & \textsf{M}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment 
        \\
    
    FChain \cite{43_Nguyen2013_FChain}
        & \textsf{M}
        & \cellcolor[HTML]{cccccc} offline anomaly detection
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment 
        \\
    ${}^\star$MicroRCA \cite{04_Wu2020_MicroRCA}
        & \textsf{M}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{S}
        & set of services
        & k8s deployment, workload generator
        \\
    ${}^\star$Wu \etal \cite{09_Wu2020_MicroserviceDiagnosisDeepLearning}
        & \textsf{M}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{S}
        & set of KPIs
        & k8s deployment, workload generator
        \\
    Sieve \cite{30_Thalheim2017_Sieve}
        & \textsf{M}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{A}
        & set of KPIs
        & target application deployment
        \\
    Brand\'on \etal \cite{11_Brandon2020_GraphBasedRootCauseAnalysis}
        & \textsf{M}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & ranked list of services
        & target application deployment, anomaly patterns
        \\
    ${}^\star$DLA \cite{14_Samir2019_DLA}
        & \textsf{M}
        & \cellcolor[HTML]{bbbbbb} topology-driven
        & \textsf{P}
        & \textsf{S}
        & set of KPIs
        & k8s deployment, application specification
        \\
    
    ${}^\star$CauseInfer \cite{40_Chen2020_CauseInfer,48_Chen2014_CauseInfer}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment
        \\
    
    ${}^\star$Microscope \cite{06_Lin2018_Microscope,19_Guan2019_MicroscopeDemo}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment
        \\
    
    ${}^\star$CloudRanger \cite{29_Wang2018_CloudRanger}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & target application deployment, historically monitored KPIs
        \\
    
    MS-Rank \cite{07_Ma2019_MSRank,25_Ma2020_MSRankExtended}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & monitored KPIs
        \\
    
    
    AutoMAP \cite{08_Ma2020_AutoMAP}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & monitored KPIs
        \\
    
    FacGraph \cite{44_Lin2018_FacGraph}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{A}
        & ranked list of services
        & monitored KPIs
        \\
    
    MicroCause \cite{05_Meng2020_RootCausesMicroservices}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{S}
        & ranked list of KPIs
        & monitored KPIs
        \\
    
    Qiu \etal \cite{46_Qiu2020_CausalityMiningKnowledgeGraph}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{S}
        & ranked list of KPIs
        & monitored KPIs, application specification
        \\
    
    ${}^\star$LOUD \cite{13_Mariani2018_LocalizingFaultsCloudSystems}
        & \textsf{M}
        & \cellcolor[HTML]{eeeeee} causality graph
        & \textsf{P}
        & \textsf{S}
        & ranked list of KPIs
        & target application deployment, workload generator
        \\
    \thickline
\end{tabular}
\end{footnotesize}
\end{table}

==> tab/rca.tex <==
\begin{table}[tp]
\caption{Classification of root cause analysis techniques, based on their \textit{class} (\viz \textsf{L}, \textsf{DT}, and \textsf{M} for log-based, distributed tracing-based, and monitoring-based techniques, respectively), the enacted \textit{search}, whether the \textit{detection} of analysed anomalies is integrated or done with external tools (\viz \textsf{I} for integrated pipelines, \textsf{E} for external tools), the \textit{type} (\viz \textsf{F} for functional anomalies, \textsf{P} for performance anomalies) and \textit{grain} of explained anomalies (\viz \textsf{A} for application-level anomalies, \textsf{S} for service-level anomalies), the identified \textit{root causes}, and the \textit{artifacts} they need to run.}
\label{tab:rca} 
\begin{footnotesize}
\begin{tabular}{%
    >{\centering\arraybackslash}m{.16\textwidth}%
    @{}
    >{\centering\arraybackslash}m{.05\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.13\textwidth}%
    >{\centering\arraybackslash}m{.14\textwidth}%
    @{\ }
    >{\centering\arraybackslash}m{.04\textwidth}%
    @{}
    >{\centering\arraybackslash}m{.06\textwidth}%
    @{}
    >{\centering\arraybackslash}m{.05\textwidth}%
    @{\,}
    >{\centering\arraybackslash}m{.11\textwidth}%
    @{\,}
    >{\centering\arraybackslash}m{.2\textwidth}%
}
    \thickline
    % study
        &
        & \multicolumn{2}{c}{\textbf{Root Cause Analysis}}
        & \multicolumn{3}{c}{\textbf{Anomaly}}
        &
        \\
    %study
        & \textbf{Class} 
        & \textbf{Approach}
        & \textbf{Method}
        & \textbf{Det.}
        & \textbf{Type}
        & \textbf{Gran.}
        & \textbf{Root Causes}
        & \textbf{Needed Artifacts}
        \\ 
    \thickline
    Aggarwal \etal \cite{10_Aggarwal2020_FaultsGoldenSignals}
        & \textsf{L}
        & \cellcolor[HTML]{FDF3ED} causality graph
        & \cellcolor[HTML]{FDF3ED} random walk 
        & \textsf{E}
        & \textsf{F}
        & \textsf{A}
        & service
        & online produced logs, application specification
        \\
    \thinline
    Zhou \etal \cite{01_Zhou2021_FaultAnalysisDebuggingMicroservices}
        & \textsf{DT}
        & \cellcolor[HTML]{D9FDE5} visualization
        & \cellcolor[HTML]{D9FDE5} trace comparison
        & \textsf{E}
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & trace events 
        & reference traces, online produced traces
        \\
    GMTA \cite{45_Guo2020_GMTA}
        & \textsf{DT}
        & \cellcolor[HTML]{D9FDE5} visualization
        & \cellcolor[HTML]{D9FDE5} trace comparison
        & \textsf{E}
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & services
        & reference traces, online produced traces
        \\
    
    CloudDiag \cite{41_Mi2013_PerformanceDiagnosisCloud}
        & \textsf{DT}
        & \cellcolor[HTML]{dfd1e6} direct
        & \cellcolor[HTML]{dfd1e6} RPCA
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment
        \\
    
    %${}^\star$
    TraceAnomaly \cite{16_Liu2020_TraceAnomaly}
        & \textsf{DT}
        & \cellcolor[HTML]{D2BBDD} direct
        & \cellcolor[HTML]{D2BBDD} KPI correlation
        & \textsf{I}
        & \textsf{F}, \textsf{P}
        & \textsf{A}
        & services
        & training traces, online produced traces
        \\
    MonitorRank \cite{21_Kim2013_RootCauseDetectionSOA}
        & \textsf{DT}
        & \cellcolor[HTML]{e8edbe} topology graph
        & \cellcolor[HTML]{e8edbe} random walk
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment
        \\
    MicroHECL \cite{47_Liu2021_MicroHECL}
        & \textsf{DT} 
        & \cellcolor[HTML]{DCE3AC} topology graph
        & \cellcolor[HTML]{DCE3AC} BFS
        & \textsf{E}
        & \textsf{P}
        & \textsf{S}
        & ranked services
        & training traces, online produced traces
        \\
    \thinline
    %${}^\star 
    $\epsilon$-diagnosis \cite{49_Shan2019_epsilonDiagnosis}
        & \textsf{M}
        & \cellcolor[HTML]{D2BBDD} direct
        & \cellcolor[HTML]{D2BBDD} KPI correlation
        & \textsf{I}
        & \textsf{P}
        & \textsf{A}
        & KPIs
        & k8s deployment
        \\
    
    %${}^\star$
    Wang \etal \cite{20_Wang2020_RootCauseMetricLocation}
        & \textsf{M}
        & \cellcolor[HTML]{D2BBDD} direct
        & \cellcolor[HTML]{D2BBDD} KPI correlation
        & \textsf{I}
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & KPIs
        & online produced logs, monitored KPIs
        \\
    PAL \cite{42_Nguyen2011_PAL}
        & \textsf{M}
        & \cellcolor[HTML]{D2BBDD} direct
        & \cellcolor[HTML]{D2BBDD} KPI correlation
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment 
        \\
    FChain \cite{43_Nguyen2013_FChain}
        & \textsf{M}
        & \cellcolor[HTML]{D2BBDD} direct
        & \cellcolor[HTML]{D2BBDD} KPI correlation
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment 
        \\
    %${}^\star$
    MicroRCA \cite{04_Wu2020_MicroRCA}
        & \textsf{M}
        & \cellcolor[HTML]{e8edbe} topology graph
        & \cellcolor[HTML]{e8edbe} random walk 
        & \textsf{I}
        & \textsf{P}
        & \textsf{S}
        & services
        & k8s deployment, workload generator
        \\
    %${}^\star$
    Wu \etal \cite{09_Wu2020_MicroserviceDiagnosisDeepLearning}
        & \textsf{M}
        & \cellcolor[HTML]{e8edbe} topology graph
        & \cellcolor[HTML]{e8edbe} random walk 
        & \textsf{I}
        & \textsf{P}
        & \textsf{S}
        & KPIs
        & k8s deployment, workload generator
        \\
    Sieve \cite{30_Thalheim2017_Sieve}
        & \textsf{M}
        & \cellcolor[HTML]{dbe0a8} topology graph
        & \cellcolor[HTML]{dbe0a8} KPI correlation
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & KPIs
        & target  app deployment
        \\
    Brand\'on \etal \cite{11_Brandon2020_GraphBasedRootCauseAnalysis}
        & \textsf{M}
        & \cellcolor[HTML]{ccd197} topology graph
        & \cellcolor[HTML]{ccd197} graph correlation
        & \textsf{E}
        & \textsf{F}, \textsf{P}
        & \textsf{S}
        & ranked services
        & target  app deployment, anomaly patterns
        \\
    %${}^\star$
    DLA \cite{14_Samir2019_DLA}
        & \textsf{M}
        & \cellcolor[HTML]{c4c98d} topology graph
        & \cellcolor[HTML]{c4c98d} HHMM
        & \textsf{I}
        & \textsf{P}
        & \textsf{S}
        & KPIs
        & k8s deployment, application specification
        \\
    %${}^\star$
    CauseInfer \cite{40_Chen2020_CauseInfer,48_Chen2014_CauseInfer}
        & \textsf{M}
        & \cellcolor[HTML]{faece3} causality graph
        & \cellcolor[HTML]{faece3} BFS 
        & \textsf{I}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment
        \\
    %${}^\star$
    Microscope \cite{06_Lin2018_Microscope,19_Guan2019_MicroscopeDemo}
        & \textsf{M}
        & \cellcolor[HTML]{faece3} causality graph
        & \cellcolor[HTML]{faece3} BFS 
        & \textsf{I}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment
        \\
    Qiu \etal \cite{46_Qiu2020_CausalityMiningKnowledgeGraph}
        & \textsf{M}
        & \cellcolor[HTML]{faece3} causality graph
        & \cellcolor[HTML]{faece3} BFS
        & \textsf{E}
        & \textsf{P}
        & \textsf{S}
        & ranked KPIs
        & monitored KPIs, application specification
        \\
    %${}^\star$
    CloudRanger \cite{29_Wang2018_CloudRanger}
        & \textsf{M}
        & \cellcolor[HTML]{FDF3ED} causality graph
        & \cellcolor[HTML]{FDF3ED} random walk 
        & \textsf{I}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & target  app deployment, historically monitored KPIs
        \\
    MS-Rank \cite{07_Ma2019_MSRank,25_Ma2020_MSRankExtended}
        & \textsf{M}
        & \cellcolor[HTML]{FDF3ED} causality graph
        & \cellcolor[HTML]{FDF3ED} random walk 
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & monitored KPIs
        \\
    AutoMAP \cite{08_Ma2020_AutoMAP}
        & \textsf{M}
        & \cellcolor[HTML]{FDF3ED} causality graph
        & \cellcolor[HTML]{FDF3ED} random walk 
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & monitored KPIs
        \\
    MicroCause \cite{05_Meng2020_RootCausesMicroservices}
        & \textsf{M}
        & \cellcolor[HTML]{FDF3ED} causality graph
        & \cellcolor[HTML]{FDF3ED} random walk 
        & \textsf{E}
        & \textsf{P}
        & \textsf{S}
        & ranked KPIs
        & monitored KPIs
        \\
    FacGraph \cite{44_Lin2018_FacGraph}
        & \textsf{M}
        & \cellcolor[HTML]{f7e7dc} causality graph
        & \cellcolor[HTML]{f7e7dc} graph correlation
        & \textsf{E}
        & \textsf{P}
        & \textsf{A}
        & ranked services
        & monitored KPIs
        \\
    %${}^\star$
    LOUD \cite{13_Mariani2018_LocalizingFaultsCloudSystems}
        & \textsf{M}
        & \cellcolor[HTML]{fae6d9} causality graph
        & \cellcolor[HTML]{fae6d9} graph centrality
        & \textsf{I}
        & \textsf{P}
        & \textsf{S}
        & ranked KPIs
        & target app deployment, workload generator
        \\
    \thickline
\end{tabular}
\end{footnotesize}
\end{table}
